OmniHD-Scenes: A Next-Generation Multimodal Dataset for Autonomous Driving

The rapid advancement of deep learning has intensified the need for comprehensive data for use by autonomous driving algorithms. High-quality datasets are crucial for the development of effective data-driven autonomous driving solutions. Next-generation autonomous driving datasets must be multimodal, incorporating data from advanced sensors that feature extensive data coverage, detailed annotations, and diverse scene representation. To address this need, we present OmniHD-Scenes, a large-scale multimodal dataset that provides comprehensive omnidirectional high-definition data. The OmniHD-Scenes dataset combines data from 128-beam LiDAR, six cameras, and six 4D imaging radar systems to achieve full environmental perception. The dataset comprises 1501 clips, each approximately 30-s long, totaling more than 450K synchronized frames and more than 5.85 million synchronized sensor data points. We also propose a novel 4D annotation pipeline. To date, we have annotated 200 clips with more than 514K precise 3D bounding boxes. These clips also include semantic segmentation annotations for static scene elements. Additionally, we introduce a novel automated pipeline for generation of the dense occupancy ground truth, which effectively leverages information from non-key frames. Alongside the proposed dataset, we establish comprehensive evaluation metrics, baseline models, and benchmarks for 3D detection and semantic occupancy prediction. These benchmarks utilize surround-view cameras and 4D imaging radar to explore cost-effective sensor solutions for autonomous driving applications. Extensive experiments demonstrate the effectiveness of our low-cost sensor configuration and its robustness under adverse conditions. Data will be released at https://www.2077ai.com/OmniHD-Scenes.

==> sections/04_benchmark.tex <==
\section{Benchmarks and Evaluation Metrics}
\label{sec:benchmark}
The OmniHD-Scenes dataset can support multiple types of tasks such as 3D detection, tracking, prediction, OCC, etc. with good extensibility due to its inclusion of a variety of sensor data and annotation information. In this paper, we introduce 3D detection and occupancy prediction tasks and evaluation metrics, and propose a novel OCC truth production process.

\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/OCC生成V2.pdf}
    % \includegraphics[width=\linewidth]{figures/框架图.pdf}
    \vspace{-0.6cm}
    \caption{Occupancy Ground Truth Generation Pipeline: we first process the key frames of the sequence with annotated LiDAR point clouds to separate dynamic objects from static elements. Tracker fake box sequences are generated for non-keyframes based on the uniform velocity assumption to enhance dynamic object features. We then use global Pose to aggregate static elements and complete semantic segmentation, and use local ICP to align dynamic objects with the same ID to reduce spatial accuracy. Finally, the noise-filtered high-density point cloud completes the voxelized representation of the occupancy state, providing detailed and reliable occupancy ground truth for autonomous driving perception.}
    \label{fig:occgt}
    \vspace{0.2cm}
\end{figure*} 
\subsection{3D Object Detection}
\label{sec:3DODAnno}
For the 3D detection task, X categories need to be detected, where each category includes a 3D box (containing the center point, length, width, height, and yaw) and velocity ($\upsilon {x}$ and $\upsilon{y}$). We refer to the evaluation metrics of the nuScenes dataset, with some simplifications and modifications.

\textbf{Average Precision (AP)}: AP is calculated using a matching method based on 2D center point distance thresholds in the Bird's Eye View (BEV) plane. As noted in the nuScenes dataset, this approach decouples the size and orientation of the target compared to Intersection over Union (IOU)-based matching methods, mitigating the bias in IOU calculations for small targets. AP is the area under the precision-recall curve, considering only recall and precision values exceeding 10\%. We set more "loose" matching thresholds of Dist={1, 2, 3, 4} to reduce the matching impact caused by the precision limitations of millimeter-wave radar, cameras, and other sensors. The AP under different distance thresholds is averaged to obtain the final AP value for a single class ccc, and the mean Average Precision (mAP) is obtained by averaging the AP values across all classes.

\textbf{True Positive Metrics (TP)}: We also provide a set of True Positive (TP) metrics for predictions matched with each ground truth (GT) box. TP metrics use a center distance of 3 meters in BEV for matching. For each class, each metric is the average of the cumulative mean values with recall rates above 10\%. Following the nuScenes methodology, we use the following TP errors:

\textbf{Average Translation Error (ATE)}: ATE is the Euclidean distance between center points in BEV.

\textbf{Average Scale Error (ASE)}: ASE is defined as 1-IOU, which represents the 3D intersection over union after aligning the center point and orientation.

\textbf{Average Orientation Error (AOE)}: AOE is the smallest angular difference between the predicted and true orientations.

\textbf{Average Velocity Error (AVE)}: AVE considers the absolute velocity error using the L2 norm of vx and vy .For each TP metric, we calculate the average across all classes, resulting in mATE, mASE, mAOE, and mAVE, which are represented overall as follows:

\textbf{OmniHD-Scenes Detection Score (ODS)}: To evaluate the overall performance of the detection model, we combine mAP with all error metrics to obtain the final overall score NOS.

The NOS final score is equally derived from the detection performance (mAP) and from quantifying the accuracy of detection in terms of bounding box position, size, orientation, and velocity. The values of mAVE, mAOE, and mATE can exceed 1, so they are limited to a range of 0-1.



\subsection{3D Semantic Occupancy}
\label{sec:OCC}
3D occupancy prediction accurately estimates the state and semantics of each position in the scene to achieve a detailed understanding of the vehicle environment. Given the lack of occupancy prediction benchmarks for surround view 4D millimeter wave radar, we design a high-quality truth generation pipeline for occupancy prediction in the OmniHD-Scenes dataset. Different from other approaches that rely on frame-by-frame panoramic segmentation of point cloud data, OmniHD-Scenes achieves occupancy truth generation by utilizing the existing 3D labeled frames and the global static scene segmentation semantics of each scene, as shown in Fig.

\subsubsection{Occupancy Ground Truth}
Single-frame LiDAR point cloud as a supervised signal for theoccupancy truth value is a fast and simple solution. However, sparse supervision from LiDAR cannot fulfill the dense scene prediction requirements.
Therefore, we efficiently aggregate sequences of LiDAR point clouds to generate dense occupancy. For key-frame point clouds, we utilize labeled 3D boxes to separate dynamic traffic participants from static elements. For unlabeled non-keyframe point clouds, based on the adjacent keyframes with uniform velocity assumption, a long-term coarse box sequence is generated and used for traffic participant information extraction.

Point clouds labeled as dynamic traffic participants were spatially transformed to frame coordinates, and then we aggregated point clouds with sequentially identical tracking IDs. Non-keyframes of dynamic traffic participants are also used for data augmentation, but simple coordinate transformations accumulate spatial alignment errors, so local ICP matching is used to eliminate interpolated frame errors during the stitching process. Each frame of static scene point cloud by global pose will be aggregated in the global coordinate system to achieve sequential scene reconstruction, and then segmentation labeling is done manually. Moreover, LIDAR generates noise points in bad scenarios such as rainy days, which are manually labeled as ignore, and the occupancy state is set to free space.

Enhanced dynamic objects and static scenes are generated by stitching together dense scene representations. Then the inverse matrix of the global pose is applied to obtain a dense point cloud for each frame. Radius filtering is applied to reduce the noise that may be present during the multi-frame stacking process.

To further densify the point cloud, many truth pipelines have attempted to achieve point cloud densification to fill in the voids using methods such as Poisson reconstruction and VBDFusion. However, the densification methods are suitable for use in low beam LIDAR, and for dense point clouds instead additional reconstruction errors are initiated leading to uneven road surfaces. Therefore, voxelization and nearest neighbor algorithms are applied to assign voxel occupancy states with semantic labels.
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/OCC可视化压缩.pdf}
    \vspace{-0.6cm}
    \caption{Multiple scenes and Semantic Occupancy visualization. From top to bottom, the images and occupancy ground truth for daytime, nighttime, and rainy scenes are displayed respectively. As can be seen, the occupancy ground truth contains richer semantic labels and clear object contours. The correspondence between colors and semantic labels can be found in Table \ref{tab:occ_performance}.}
    \label{fig:OCC-Vis}
    \vspace{0.2cm}
\end{figure*}  
\subsubsection{Occupancy Metrics}

For 3D occupancy prediction performance metrics are organized around occupancy state with semantic segmentation. For each category we use Intersection of Union (IoU) [Semantickitti] as semantic metric. In addition, mIoU is the average of all categories of IoU reflecting the combined performance. The calculation formula is as follows.

\begin{equation}
    \mathrm{IoU} =\frac{T P}{T P+F P+F N}
\end{equation}
\begin{equation}
    \mathrm{mIoU} = \frac{1}{C} \sum_{i = 1}^{C} \frac{T P_{i}}{T P_{i}+F P_{i}+F N_{i}}
\end{equation}

where TP, FP, FN indicate the number of true positive, false positive, and false negative predictions. C is the number of categories without free space. Further, we evaluate the accuracy of the occupancy state estimation. Scene completion IoU (SC IoU) is used to specifically evaluate geometric metrics, statistically computing free space and non-empty elements similar to IoU.




==> sections/06_analysis.tex <==
\section{Analysis and Discussion}
\label{sec:dis}
This section delves into the nuanced relationships between model designs and robustness under various corruptions. Subsection~\ref{sec:depth} explores the performance of depth estimation models and highlights their susceptibility to image corruptions. Subsection~\ref{sec:pretrain} discusses the impact of pre-training on model resilience across different corruptions. Subsection~\ref{sec:temporal} examines the benefits of temporal fusion. Subsection~\ref{sec:backbone} compares the robustness of different model backbones. Subsection~\ref{sec:corrupt-ana} analyzes how pixel distribution changes correlate with model performance under corruption. Finally, Subsection~\ref{sec:detail-metric} provides detailed metrics on how specific model errors.


\begin{figure*}[ht]
    \centering
    \subfloat[Pre-train - mCE]{
        \label{fig:nds-mce-pretrain}
        \includegraphics[width=0.232\linewidth]{figures/mce-nds-pretrain.pdf}
    }
    ~~
    \subfloat[Pre-train - mRR]{
        \label{fig:nds-mrr-pretrain}
        \includegraphics[width=0.232\linewidth]{figures/mrr-nds-pretrain.pdf}
    }
    ~~
    \subfloat[Depth - mCE]{
        \label{fig:nds-mce-depth}
        \includegraphics[width=0.232\linewidth]{figures/mce-nds-depth.pdf}
    }
    ~~
    \subfloat[Depth - mRR]{
        \label{fig:nds-mrr-depth}
        \includegraphics[width=0.232\linewidth]{figures/mrr-nds-depth.pdf}
    }
    \label{fig:pretrain}
    \vspace{-0.1cm}
    \caption{Ablation study. We observe that pre-training strategies together with depth-free bird's eye view transformation provide the models with better robustness. We do not consider SOLOFusion \cite{Park2022TimeWT} long-term fusion here since it utilizes 16 frames, which is much larger than other methods.}
    \vspace{-0.2cm}
\end{figure*}


\begin{figure*}[t]
    \centering
    \subfloat[Camera Crash - CE]{
        \label{fig:nds-mce-cam-temp}
        \includegraphics[width=0.23\linewidth]{figures/mce-nds-cam-temporal.pdf}
    }
    ~~
    \subfloat[Camera Crash - RR]{
        \label{fig:nds-mrr-cam-temp}
        \includegraphics[width=0.23\linewidth]{figures/mrr-nds-cam-temporal.pdf}
    }
    ~~
    \subfloat[Frame Lost - CE]{
        \label{fig:nds-mce-frame-temp}
        \includegraphics[width=0.23\linewidth]{figures/mce-nds-frame-temporal.pdf}
    }
    ~~
    \subfloat[Frame Lost - RR]{
        \label{fig:nds-mrr-frame-temp}
        \includegraphics[width=0.23\linewidth]{figures/mrr-nds-frame-temporal.pdf}
    }
    \vspace{0.cm}
    \caption{Ablation study. We observe that not all the models with temporal fusion exhibit better robustness under \textit{Camera Crash} and \textit{Frame Lost}. However, they have exhibited certain potential since models with the lowest mCE metric are always those that utilize temporal information.}
    \label{fig:temporal}
\end{figure*}


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/fig_backbone.png}
    \vspace{-0.6cm}
    \caption{Backbone comparison: ResNet \cite{he2016deep} \textit{vs.} VoVNet-V2 \cite{lee2020centermask}. We compare the absolute corruption error (\textit{i.e.}, CE) since the two variants have similar ``clean'' performances.}
    \label{fig:backbone}
\end{figure}


\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/fig_swint.png}
    \vspace{-0.6cm}
    \caption{Backbone comparison: ResNet \cite{he2016deep} \textit{vs.} Swin Transformer \cite{liu2021swin}. We compare the relative corruption error (\textit{i.e.}, RR) since the two variants have different ``clean'' performances.}
    \label{fig:swin-backbone}
\end{figure}


\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/fig_pretrain.png}
    \vspace{-0.6cm}
    \caption{Pre-training comparisons. We compare the resilience rate (RR) between BEVDet~\cite{huang2021bevdet} with and without using model pre-training.}
    \label{fig:bevdet-pretrain}
\end{figure}


\subsection{Depth Estimation}
\label{sec:depth}
- \textit{Depth-free BEV transformations show better robustness.}
Our analysis reveals that depth-based approaches suffer from severe performance degradation when exposed to corrupted images as shown in Figure~\ref{fig:nds-mce-depth} and~\ref{fig:nds-mrr-depth}. Moreover, we undertake a comparative study to evaluate the intermediate depth estimation results of BEVDepth~\cite{li2022bevdepth} under corruptions. To this end, we compute the mean square error (MSE) between ``clean'' inputs and corrupted inputs. Our findings indicate an explicit correlation between vulnerability and depth estimation error, as presented in Figure~\ref{fig:bevdepth-depth-error}. Specifically, \textit{Snow} and \textit{Dark} corruptions significantly affect accurate depth estimation, leading to the largest performance drop. These results provide further support for our conclusion that the performance of depth-based approaches can suffer significantly if the depth estimation is not accurate enough. The depth estimation results under corruptions can be seen from Figure~\ref{fig:depth-estimation}, where we can see significant differences under certain corruptions (\textit{e.g.}, \textit{Snow}) compared to ``clean'' inputs.


\input{tables/stat3d}


\subsection{Model Pre-Training}
\label{sec:pretrain}
- \textit{Pre-training improves robustness across a wide range of semantic corruptions while does not help with temporal corruptions.} The effectiveness of these strategies for improving model robustness is illustrated in Figure~\ref{fig:nds-mce-pretrain} and Figure~\ref{fig:nds-mrr-pretrain}, where models that utilize pre-training largely outperform those not. For controlled comparison, we re-implement the BEVDet (r101)~\cite{huang2021bevdet} model using the FCOS3D~\cite{wang2021fcos3d} checkpoint as initialization. Our results, presented in Figure~\ref{fig:bevdet-pretrain}, show that pre-training can significantly improve mRR across a wide range of corruptions (except \textit{Fog}) even if it has lower ``clean'' NDS (0.3780 \textit{vs.} 0.3877). Specifically, under \textit{Color Quant}, \textit{Motion Blur}, and \textit{Dark} corruptions, the mRR metric improves by 22.5\%, 17.2\%, and 27.8\%, respectively. It is worth noting that pre-training mainly improves most semantic corruptions and does not improve temporal corruptions. Even though, the pre-trained BEVDet still largely lags behind those depth-free counterparts. Therefore, we can conclude that pre-training together with the depth-free bird's eye view transformation provides models with strong robustness. More recently, M-BEV~\cite{chen2024m} propose masked pre-training task to enhance robustness under incomplete sensor input. We compare a masked pre-trained PETR with the corresponding baseline. The results can be seen in Table~\ref{tab:mbev}. We find M-BEV can most effectively improve robustness towards incomplete sensor output, and reveal the promise of masked image modeling pre-train in BEV perception tasks.


\subsection{Temporal Fusion}
\label{sec:temporal}
- \textit{Temporal fusion has the potential to yield better absolute performance under corruptions. Fusing longer temporal information largely helps with robustness.}
We are particularly interested in examining how models utilizing temporal information perform under temporal corruptions. We find SOLOFusion~\cite{Park2022TimeWT} which fuses wider and richer temporal information performs extremely well compared to its short-only and long-only versions. In terms of \textit{Camera Crash}, the short-only and long-only versions have close resilience rate performance (65.04 \textit{vs.} 65.13). However, the fusion version improves to 70.73, which is the highest among all the candidate models. Similarly, the fusion version improves the resilience rate by almost 10\%  compared to the other two versions under \textit{Frame Lost} corruption. Moreover, the RR metric of its long-only version outperforms its short-only counterpart on a wide range of corruption types, which indicates the great potential of utilizing longer temporal information.



\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/error_plot.pdf}
    \vspace{-0.6cm}
    \caption{Visualized feature errors between the corruption inputs and the ``clean'' inputs. We observe that temporal fusion exhibits a certain potential to mitigate the noises caused by corrupted input images.}
    \label{fig:temp-error}
\end{figure}




To further investigate the impact of temporal fusion on enhancing the corruption robustness, we employ the BEVFormer model to assess feature errors with and without the integration of temporal information compared to ``clean'' temporal inputs. We compute the mean squared error (MSE) between corrupted inputs, both with and without temporal information, and ``clean'' inputs with temporal information. The results are shown in Figure~\ref{fig:temp-error}. We note a trend of increasing error over time in the temporal fusion model (illustrated by the blue bar), attributable to error accumulation under consecutive corrupted inputs. Despite this, temporal fusion consistently demonstrates an error mitigation effect across frames.


However, we find that not all models with temporal fusion exhibit better robustness under \textit{Camera Crash} and \textit{Frame Lost}. The robustness is highly correlated to how to fuse history frames and how many frames are used, which emphasizes the importance of evaluating temporal fusion strategies from wider perspectives. The results can be seen in Figure~\ref{fig:temporal}. Nonetheless, temporal fusion remains a potential method to enhance temporal robustness since the models with the lowest Corruption Error (or the highest Resilience Rate) are consistently those that utilize temporal information.

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{figures/visualization_main.pdf}
    \caption{Visualizations of detection results from BEVFormer~\cite{li2022bevformer}. From left to right: top: GT, \textit{Clean}, \textit{Motion}, \textit{Quant}; bottom: \textit{Bright}, \textit{Dark}, \textit{Fog}, \textit{Snow}.}
    \label{fig:visual}
\end{figure*}

\subsection{Backbone}
\label{sec:backbone}
- \textit{The Swin Transformer is more vulnerable towards the lighting changings; VoVNet-V2 is more robust against Snow while ResNet shows better robustness across a wide range of corruptions.} Although ResNet~\cite{he2016deep} and VoVNet~\cite{lee2020centermask} exhibit close standard performance, ResNet-based detectors exhibit consistently superior robustness across a wide range of corruptions, as illustrated in Figure~\ref{fig:backbone}.
Conversely, the VoVNet backbone consistently exhibits better robustness under \textit{Snow} corruptions. Moreover,  Swin Transformer~\cite{liu2021swin} based BEVDet~\cite{huang2021bevdet} demonstrates significant vulnerability towards changes in lighting conditions (\textit{e.g.}, \textit{Bright} and \textit{Dark}). A clear comparison can be found in Figure~\ref{fig:swin-backbone}. Inspired by~\cite{johnson2016perceptual}, we compute the Gramian matrix in the feature space in the features extracted by the backbone model, under benign inputs and corruption inputs. Based on that, we compute the relative error between the ``clean'' and corruption inputs Gramian matrix. The VoVNet has a relative error of 4.17 and 5.43 towards \textit{Snow} and \textit{Motion Blur}, respectively. While ResNet has errors of 11.47 and 2.10. The results align with our end-to-end experiments above, where ResNet is more robust under \textit{Motion Blur} while VoVNet is more robust towards \textit{Snow}. The observed robustness differences between ResNet and VoVNet to \textit{Snow} and \textit{Motion Blur} stem from their architectural designs. ResNet's deep hierarchical features and skip connections make it more sensitive to high-frequency noise like \textit{Snow}, resulting in higher errors. Conversely, VoVNet's dense feature aggregation and efficient feature use enhance robustness to \textit{Snow} by mitigating local noise patterns. However, VoVNet shows higher errors under \textit{Motion Blur}. ResNet's hierarchical feature representation might be better suited to handling the spatial inconsistencies caused by simulated \textit{Motion Blur}. These findings suggest VoVNet excels in spatial noise resilience, while ResNet handles spatial distortions better. Furthermore, the finding can provide insights for feature work to design new loss functions towards aligning the Gramian matrix of features extracted by backbone under different corruptions.


\subsection{Corruptions}
\label{sec:corrupt-ana}
\textit{The relationship between pixel distribution shifts and model performance degradation is not straightforward.}
We calculate the pixel distribution over 300 images sampled from the nuScenes dataset and visualize the pixel histograms shown in Figure~\ref{fig:hist}. Interestingly, the \textit{Motion Blur} causes the least pixel distribution shifts while causing a relatively large performance drop. On the other hand, \textit{Bright} shifts the pixel distribution to higher values, and \textit{Fog} makes fine-grained features more indistinct by shifting the pixel value more agminated. However, these two corruptions only lead to the smallest performance gap, which reveals that model robustness is not simply correlated with pixel distribution.


\subsection{Detailed Metrics}
\label{sec:detail-metric}
- \textit{Velocity prediction errors amplify under corruptions, and attribution and scale errors differ across models.}
While our study predominantly reports the nuScenes Detection Score (NDS) metrics, additional insights into model robustness are illustrated in Figure~\ref{fig:stat-3d}. We find that models incorporating temporal information, such as BEVFormer~\cite{li2022bevformer} and BEVerse~\cite{zhang2022beverse}, exhibit substantially lower mean Absolute Velocity Error (mAVE) compared to those that do not. Nonetheless, even models with temporal fusion are not immune to the adverse effects of image corruption; specifically, velocity prediction errors markedly escalate even under mild illumination alterations. Figure~\ref{fig:3d-bevformer} and \ref{fig:3d-beverse} illustrates that \textit{Motion Blur} corruption detrimentally influences the velocity predictions for both BEVFormer and BEVerse, revealing a significant vulnerability in these models that incorporate temporal data.
Moreover, a closer examination of attribution and scale errors reveals considerable heterogeneity across models. Depth-free models demonstrate a consistent performance in these metrics, while depth-based models display pronounced variability. This observation underscores the heightened susceptibility of depth-based methods to image corruptions and emphasizes the need for further research to enhance their robustness. 

